Revisiting Offline Compression: Going Beyond Factorization-based Methods for Transformer Language Models

Recent transformer language models achieve outstanding results in many natural language processing (NLP) tasks. However, their enormous size often makes them impractical on memory-constrained devices, requiring practitioners to compress them to smaller networks. In this paper, we explore offline compression methods, meaning computationally-cheap approaches that do not require further fine-tuning of the compressed model. We challenge the classical matrix factorization methods by proposing a novel, better-performing autoencoder-based framework. We perform a comprehensive ablation study of our approach, examining its different aspects over a diverse set of evaluation settings. Moreover, we show that enabling collaboration between modules across layers by compressing certain modules together positively impacts the final model performance. Experiments on various NLP tasks demonstrate that our approach significantly outperforms commonly used factorization-based offline compression methods.

==> background.tex <==
\section{Related Work}
\label{sec:background}



==> outline.tex <==
checking the direction for other wegiht matrices than token embedding

grid search on e.g. keys module

ablation study on linear vs non-linear reconstruction modules

enforcing norm ablation study
    embeddings
    keys/query/value (not yet there)
    
sensitivity experiments
    fischer weights being 
    the way sensitivity is implemented
    different transformation on sensitivity scores
    
drone experiment
    key/query/value/FFs
    effect of drone coeff
    effect of drone on perplexity stability/final value
    effect of drone on down-stream task (not yet there) --> use latest master code
    
kronecker/tucker insights
    discussing on why tensor-decomposition appraoches perform as similar as random inits
    the whole work is done by distillation in previous work
    

main question:
    how to do the offline compression most efficient, so that we dont rely heavily on expensive distillation-based approaches

baseline to compare with
    SVD in most scenarios
    emphasize why SVD is chosen (probably because it's optimal for linear model that are L2 based in training)

concatenated/separated idea
    idea of layers collaborating together instead of being trained separately (key/query/value/FFs) --> 
    
performance when all ideas are merged

==> tables/temp_final_table.tex <==
\begin{table*}[h!]
    \small
    \centering
    \vskip 0.1in
    % \begin{tabular}{@{}c@{\;}cccccc}
    \begin{tabular}{@{}ccrrlrrlrrl@{}}
                 
         \toprule
         CR & Architecture & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}MRPC\\ (F1/Acc)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}SST-2 \\ (Acc)\end{tabular}}  & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}RTE \\(Acc)\end{tabular}}  & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}QNLI \\ (Acc)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}QQP \\ (F1/Acc)\end{tabular}}\\
         \midrule
         
         % CR & Architecture & \makecell{MRPC \\ (F1/Acc)} & \makecell{SST-2 \\ (Acc)} & \makecell{RTE \\ (Acc)} & \makecell{QNLI \\ (Acc)} & \makecell{QQP \\ (F1/Acc)} \\
         % \midrule
         
         1 & BERT$_{BASE}$ &  88.85/84.07 & 92.32 & 65.70	 & 90.66 & 87.49/90.71 \\ 
         \midrule
         
        \multirow{2}{*}{\begin{tabular}[x]{@{}c@{}}3\end{tabular}}
         & SVD & 84.35/77.45 & 86.70 & 62.09 & 85.61 & 84.64/88.38 \\
         & Our & \textbf{85.25/77.77} & \textbf{90.25} & \textbf{62.45} & \textbf{88.68} & \textbf{86.07/89.71}\\
         \midrule
         
         \multirow{2}{*}{\begin{tabular}[x]{@{}c@{}}10\end{tabular}}
         & SVD & 78.46/68.38 & 82.00 & 52.71 & 77.48 & 79.36/83.45\\
         % & Our & \textbf{80.20/70.34} & \textbf{83.94} & \textbf{57.76} & \textbf{81.48} \\
          & Our & \textbf{81.45/71.08} & \textbf{83.94} & \textbf{57.76} & \textbf{81.48} & \textbf{81.57/85.75}\\
         \midrule
         
         \multirow{2}{*}{\begin{tabular}[x]{@{}c@{}}25\end{tabular}}
         & SVD & 77.10/66.42 & 78.33 & 53.43 & 62.66  & 74.21/79.10\\
         % & Our & \textbf{78.07/68.14} & \textbf{80.05} &  \textbf{55.23} & \textbf{72.96} \\
         & Our & \textbf{81.60/71.32} & \textbf{80.05} &  \textbf{55.23} & \textbf{72.96} & \textbf{78.45/83.11}\\
         \bottomrule
    \end{tabular}
    \caption{Final BERT$_{BASE}$ model compression (token embedding matrix, all key matrices, and all output-dense matrices). The baseline SVD algorithm compresses each matrix separately. Our autoencoder-based approach, incorporates mechanisms developed in the ablation study presented in this work (see~\Cref{tab:appendix:ae_hyperparameters} for the detailed AE design choices). For each setting, we present the median score from experiments with three different seeds. Our approach consistently outperforms the classical factorization method.}
    
    % median from 3 different seeds, SVD (separated) vs our approach, token embeddings, self-attention (key,query,value,attention output), intermediate dense, output-dense.}
    \label{tab:fullbertcompression}
\end{table*}

